EasyTrack: Efficient and Compact One-stream 3D Point Clouds Tracker

Most of 3D single object trackers (SOT) in point clouds follow the two-stream multi-stage 3D Siamese or motion tracking paradigms, which process the template and search area point clouds with two parallel branches, built on supervised point cloud backbones. In this work, beyond typical 3D Siamese or motion tracking, we propose a neat and compact one-stream transformer 3D SOT paradigm from the novel perspective, termed as \textbf{EasyTrack}, which consists of three special designs: 1) A 3D point clouds tracking feature pre-training module is developed to exploit the masked autoencoding for learning 3D point clouds tracking representations. 2) A unified 3D tracking feature learning and fusion network is proposed to simultaneously learns target-aware 3D features, and extensively captures mutual correlation through the flexible self-attention mechanism. 3) A target location network in the dense bird's eye view (BEV) feature space is constructed for target classification and regression. Moreover, we develop an enhanced version named EasyTrack++, which designs the center points interaction (CPI) strategy to reduce the ambiguous targets caused by the noise point cloud background information. The proposed EasyTrack and EasyTrack++ set a new state-of-the-art performance ($\textbf{18\%}$, $\textbf{40\%}$ and $\textbf{3\%}$ success gains) in KITTI, NuScenes, and Waymo while runing at \textbf{52.6fps} with few parameters (\textbf{1.3M}). The code will be available at https://github.com/KnightApple427/Easytrack.

==> README <==
README
------

  The subfigure package has been superseded by the subfig package.
  The reason for the name change is that the new subfig package is not
  exactly backward compatible with this package; although, it comes
  with a configuration file that *almost* allows backward
  compatibility, the difference is that exact spacing and layout of
  the subfloats are not preserved.

  The newer (subfig) package is an improvement over this package and
  although this package will continue to be supported, it will no longer
  be updated.

This directory contains version 2.1.5 of the subfigure package.
Use `make' to extract the subfigure package and run the local tests.

MANIFEST:
---------
Makefile           UNIX makefile to extract the subfigure package
                       and related material.
README             This file.
subfigure.dtx      The documented subfigure package.
subfigure.ins      The subfigure package installation file.
subfigure.pdf      Subfigure package documentation (as PDF).
test.tex           Test one: Mixed tables and figures.
test2.tex          Test two: Check for extra space around figure
test3.tex          Test four: Test of optional args and \subref.
test4.tex          Test four: Test of interaction with hyperref.
test5.tex          Test five: Test for class \let of \endfigure, etc.

FILES AFTER `make':
-------------------
Makefile           UNIX makefile to extract the subfigure package
                       and related material.
README             This file.
ltxdoc.cfg         Configuration file to print change history and
                       index on the subfigure package documentation.       
subfigure.cfg      Set the preferred options for subfigure version 2.1.
subfigure.dtx      The documented subfigure package.
subfigure.ins      The subfigure package installation file.
subfigure.pdf      Subfigure package documentation (as PDF).
subfigure.ps       Subfigure package documentation (as PostScript).
subfigure.sty      The subfigure package 
test.ps            Results of test one.
test.tex           Test one: Mixed tables and figures.
test2.ps           Results of test two.
test2.tex          Test two: Check for extra space around figure
test3.ps           Results of test three.
test3.tex          Test four: Test of optional args and \subref.
test4.pdf          Results of test four.
test4.tex          Test four: Test of interaction with hyperref.
test5.tex          Test five: Test for class \let of \endfigure, etc.
test5a.ps          Results of test five (log file).
test5b.ps          Results of test five (output).

NOTES:
------

By default, the subfigure.sty file acts like the older versions of the
subfigure package.  To make the preferred options default move the
subfigure.cfg file into the standard TEXINPUTS path along with the
subfigure.sty file.  This reduces the whitespace around the subfigures
and subtables and sets the table style to have the captions and
subcaptions preceed the table and subtables.

